PAC-Bayesian Majority Vote for Late Classifier Fusion

A lot of attention has been devoted to multimedia indexing over the past few years. In the literature, we often consider two kinds of fusion schemes: The early fusion and the late fusion. In this paper we focus on late classifier fusion, where one combines the scores of each modality at the decision level. To tackle this problem, we investigate a recent and elegant well-founded quadratic program named MinCq coming from the Machine Learning PAC-Bayes theory. MinCq looks for the weighted combination, over a set of real-valued functions seen as voters, leading to the lowest misclassification rate, while making use of the voters' diversity. We provide evidence that this method is naturally adapted to late fusion procedure. We propose an extension of MinCq by adding an order- preserving pairwise loss for ranking, helping to improve Mean Averaged Precision measure. We confirm the good behavior of the MinCq-based fusion approaches with experiments on a real image benchmark.

==> barre.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2058,840){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(2058,1579){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(2058,2318){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%
      \put(2058,3057){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%
      \put(2058,3796){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%
      \put(2058,4535){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%
      \put(2310,420){\makebox(0,0){\strut{}aeroplane}}%
      \csname LTb\endcsname%
      \put(2568,420){\makebox(0,0){\strut{}bicycle}}%
      \csname LTb\endcsname%
      \put(2827,420){\makebox(0,0){\strut{}bird}}%
      \csname LTb\endcsname%
      \put(3085,420){\makebox(0,0){\strut{}boat*}}%
      \csname LTb\endcsname%
      \put(3343,420){\makebox(0,0){\strut{}bottle}}%
      \csname LTb\endcsname%
      \put(3602,420){\makebox(0,0){\strut{}bus*}}%
      \csname LTb\endcsname%
      \put(3860,420){\makebox(0,0){\strut{}car}}%
      \csname LTb\endcsname%
      \put(4118,420){\makebox(0,0){\strut{}cat}}%
      \csname LTb\endcsname%
      \put(4377,420){\makebox(0,0){\strut{}chair*}}%
      \csname LTb\endcsname%
      \put(4635,420){\makebox(0,0){\strut{}chair-dinning}}%
      \csname LTb\endcsname%
      \put(4893,420){\makebox(0,0){\strut{}cow}}%
      \csname LTb\endcsname%
      \put(5151,420){\makebox(0,0){\strut{}dinningtable*}}%
      \csname LTb\endcsname%
      \put(5410,420){\makebox(0,0){\strut{}dog}}%
      \csname LTb\endcsname%
      \put(5668,420){\makebox(0,0){\strut{}horse*}}%
      \csname LTb\endcsname%
      \put(5926,420){\makebox(0,0){\strut{}motorbike*}}%
      \csname LTb\endcsname%
      \put(6185,420){\makebox(0,0){\strut{}person}}%
      \csname LTb\endcsname%
      \put(6443,420){\makebox(0,0){\strut{}pottedplant}}%
      \put(336,2687){\rotatebox{-270}{\makebox(0,0){\strut{}MAP}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4616,4262){\makebox(0,0)[r]{\strut{}MinCQ}}%
      \csname LTb\endcsname%
      \put(4616,3842){\makebox(0,0)[r]{\strut{}MinCQ$_{avgmap}$}}%
      \csname LTb\endcsname%
      \put(4616,3422){\makebox(0,0)[r]{\strut{}MinCQ$_{avgmap}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{barre}}%
    \gplfronttext
  \end{picture}%
\endgroup

